Pairwise Link Prediction

Link prediction is a common problem in network science that transects many disciplines. The goal is to forecast the appearance of new links or to find links missing in the network. Typical methods for link prediction use the topology of the network to predict the most likely future or missing connections between a pair of nodes. However, network evolution is often mediated by higher-order structures involving more than pairs of nodes; for example, cliques on three nodes (also called triangles) are key to the structure of social networks, but the standard link prediction framework does not directly predict these structures. To address this gap, we propose a new link prediction task called "pairwise link prediction" that directly targets the prediction of new triangles, where one is tasked with finding which nodes are most likely to form a triangle with a given edge. We develop two PageRank-based methods for our pairwise link prediction problem and make natural extensions to existing link prediction methods. Our experiments on a variety of networks show that diffusion based methods are less sensitive to the type of graphs used and more consistent in their results. We also show how our pairwise link prediction framework can be used to get better predictions within the context of standard link prediction evaluation.

==> 005-01-synthetic.tex <==
\subsection{Synthetic experiments}
In this set of experiments, we use both preferential
attachment and stochastic block model
networks, and generate graphs of $600$ nodes as input to the wedges and 80-20
experiments. 

\xhdr{Generalized Preferential Attachment (GPA)}
%
Generalized Preferential Attachment~\cite{Avin-GPA-2017} is a graph generation
model that generalizes the classical preferential attachment
model~\cite{Newman-growing-networks-2001}, to allow for the addition of
new components at each step of the algorithm, and not just nodes. In our generation
of synthetic graphs, we allow the event of node addition with probability $1/2$,
and we allow the event of edge addition with probability $1/2$. The starting
graph structure is a clique of size 5. At each step of the graph generation
process, an edge or node is added by attaching proportionally to the degrees of
the existing nodes.

\xhdr{Stochastic Block Model (SBM)}
%
In this model, we plant three communities of size $200$ nodes
each, and set the edge probability within each community to be $20/200$, and the
edge probability between any two communities to be $10/200$.  When testing our
methods on the SBM model, we keep the connections within communities and only
hide edges across communities to be predicted. In the \textit{wedges experiment},
we only select edges between two communities and find their
corresponding third node to form triangles with from the third community.

\xhdr{Results}
%
Figures~\ref{fig:synthetic-wedge-edge} and~\ref{fig:synthetic8020} show the
results of the pairwise link prediction for the wedges experiments and 80-20
experiments, respectively.  In all experiments, our pair-seeded PageRank and
TRPR methods produce better results than the single seeded method and the local
similarity measures. For the results in Figure~\ref{fig:synthetic-wedge-edge} with the GPA model, the
setup of the wedges experiment forces the constraint that any edge $(u, v)$ used
for prediction participates in no triangles in the training data. Thus,
$\Gamma((u, v))$ is empty and the local methods evaluate to zero. In the
SBM experiment, we only removed certain types of edges, so the local methods do
not always evaluate to zero.

As expected, the results in Figure~\ref{fig:synthetic8020}
for the PA baseline makes many good predictions on the GPA graph, with the
median close to 1.  This is not a surprise since the GPA graph model builds the
graph by appending new nodes or edges to existing nodes with probability
proportional to the degrees of the existing nodes.

% OLD FIGURES
\hide{
\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{synthetic/a_synthetic_wedges_edges}
  \caption{Box plots of the AUC scores distribution from the wedges experiment applied on synthetic graphs under the GPA (top panel) and SBM (bottom panel) models. The numbers are the median value. Pair-seeded PageRank and TRPR are our proposed methods for pairwise link prediction and they are consistently better than other single seeded PageRank and the local similarity metrics. See the discussion in the text about AA, PA, and JS on the GPA experiment. }
  \label{fig:synthetic-wedge-edge}
\end{figure}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{synthetic/a_synthetic_80_20}
  \caption{Box plots of the AUC scores distribution from the 80-20 experiment. The numbers are the median value.  In both scenarios, GPA (top panel) and SBM (bottom panel), we observe that pair-seeded PageRank and TRPR are superior to other methods.}
  \label{fig:synthetic8020}
\end{figure}
}

%%% Old version
\hide{
\subsection{Synthetic experiments}
In this set of experiments, we use two kinds of synthetically generated networks, and generate graphs of size $600$ nodes in each of the models below. 

\xhdr{Stochastic Block Model (SBM)} In the stochastic block model, we plant communities of size $200$ nodes each, and set the density of each community to be $10/200$, and the density of the bipartite connections between any two communities to be $10/200$. When testing our methods on the SBM model, we keep the connections within communities and only hide edges across communities to be predicted. For instance, in the \textit{wedges experiment}, we only select edges between two communities and find their corresponding third node to form triangles with from the third community.

\xhdr{Generalized Preferential Attachment (GPA)} Generalized Preferential Attachment~\cite{Avin-GPA-2017} is a graph generation model that generalizes the classical preferential attachment model~\cite{Newman-growing-networks-2001}, to allow for the addition of components at each step of the algorithm, and not just nodes. In our synthetic graphs generation, we allow the event of node addition with probability $1/2$, and we allow the event of edge addition with probability $1/2$. The starting graph structure is a clique of size 5.

%\xhdr{Triangle dense graph (TDG)} The graph we use here is a clique of size $600$, and the triangle density of this graph is equal to $1$. This graph serves the purpose 
%The purpose of using such graph is to identify one extreme scenario under which collapsing the network proves to be the most useful.

We show the results of the synthetic experiments in Figures~\ref{fig:synthetic-wedge-edge} and~\ref{fig:synthetic8020}. In all experiments, we can observe that pair-seeded PageRank or TRPR produce better results than the single seeded answer. They also consistently produce better results than the local similarity measures. Note that in Figure~\ref{fig:synthetic-wedge-edge}, the local measures evaluate to zero on the GPA graphs since the set $\Gamma(e)$ where $e$ is as seed node is empty, and evaluate to nonzero in the SBM model since we keep the edges within the communities. One interesting, and expected, observation from Figure~\ref{fig:synthetic8020} is that the PA metric makes many good predictions on the GPA graph, with the median being close to 1. This is not a surprise since the GPA graph model builds the graph by appending new nodes or edges to existing nodes with probability proportional to the degrees of the existing nodes.
\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{synthetic/a_synthetic_wedges_edges}
  \caption{Box plots of the AUC scores distribution from the wedges experiment applied on synthetic graphs under the GPA (top panel) and SBM (bottom panel) models. Pair-seeded PageRank and TRPR are our proposed methods for pairwise link prediction and they are consistently better than other single seeded PageRank and the local similarity metrics.}
  \label{fig:synthetic-wedge-edge}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{synthetic/a_synthetic_80_20}
  \caption{Box plots of the AUC scores distribution from the 80-20 experiment. The small inset figure in the top panel is a zoom-in on the values from 0.9 to 1 for the first 4 methods. In both scenarios, GPA (top panel) and SBM (bottom panel), we observe that pair-seeded PageRank and TRPR aser superior to other methods.}
  \label{fig:synthetic8020}
\end{figure}
}


==> 005-02-real.tex <==
\subsection{Real-world graphs}
\label{sec:real-world}
In this section we perform our pairwise link prediction experiments
on six real-world graphs from different domains. The networks are as follows:
\begin{itemize}
\item Penn94, MU78, and Caltech36 are online social networks from
  the Facebook100 collection of datasets~\cite{Traud-facebook100-2011}.
\item Ch-Ch-Miner is a biological network of drug (chemical) interactions~\cite{Wishart-drugbank-2017,biosnapnets}.
\item P-P-Pathways is a biological network of  physical interactions between proteins in humans~\cite{Agrawal-PPI-2018}.
\item email is an email communication network~\cite{Guimer-selfsimilar-2003}.
\end{itemize}
Table~\ref{tab:datasets} provides summary statistics for these datasets,
along with the temporal network we use in the next section. 



Figure~\ref{fig:real-wedges-edges} shows the results of the wedges experiments.
Recall that the baseline measures do not produce meaningful output for this
experiment. 
Again, we see that pair-seeded PageRank and TRPR consistently produce better
performance as compared to single seeded PageRank.  The results of the 80-20
experiments for the online social networks are in Figure~\ref{fig:facebook100}.
Here, we observe an improvement of the local methods such as Adamic-Adar and
Jaccard Similarity. Nevertheless, this is not unexpected, as these metrics model
the social interactions paradigm such as having a large number of common friends.
We show the 80-20 experiment on the remaining networks
in Figure~\ref{fig:nonfacebook}. The one scenario in which a local method
outperforms the diffusion methods is the protein-protein interaction network
where the PA metric produces the best performance. This might not be surprising,
as studies have suggested that preferential attachment governs the evolution of
protein-protein interaction
networks~\cite{Eisenberg-PPIprefattach-2003}.

\hide{
\begin{figure}[t]
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.49\linewidth]{real-wedges-edges/a_Penn94_wedge_edge}%
    \includegraphics[width=0.49\linewidth]{real-wedges-edges/a_CC_wedge_edge}%
  \end{minipage}\\
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.49\linewidth]{real-wedges-edges/a_MU_wedge_edge}%
    \includegraphics[width=0.49\linewidth]{real-wedges-edges/a_PP_wedge_edge}%
  \end{minipage}\\
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.49\linewidth]{real-wedges-edges/a_caltech_wedges_edges}%
    \includegraphics[width=0.49\linewidth]{real-wedges-edges/a_email_wedges_edges}%
  \end{minipage}
  \caption{Results of the wedges experiment on six real-world networks from
    Table~\ref{tab:datasets}. Pair-seeded PageRank and TRPR produce superior
    results as compared to single-seeded PageRank in all experiments.}
  \label{fig:real-wedges-edges}
\end{figure}}

%\begin{figure}
%  \begin{minipage}{0.3\linewidth}
%    \includegraphics[width=\linewidth]{couple}
%  \end{minipage}
%  \begin{minipage}{0.6\linewidth}
%    \caption{Motivating social network example for the TRPR algorithm. If all of the
%      \textit{friends} of the blue couple know the red node, we want to
%      predict that the red node must know the blue couple as well. Running
%      TRPR on the above example, with $\ve_{u,v}$ being a seed vector on the
%      blue nodes reveals the red node being the third highest score after
%      the two blue nodes. After $10$ iterations of Algorithm~\ref{alg:trpr} with
%      $\alpha = 0.8$, the ouput vector assigns a score of $0.102$ to the red node,
%      $0.063$ to the black nodes, and $0.257$ to the blue nodes.}
%    \label{fig:trpr}
%  \end{minipage}
%\end{figure}




% OLD FIGURES
\hide{
\begin{fullwidth} 
\begin{figure}
  \begin{minipage}{\dimexpr(\textwidth+\marginparwidth)}
    \includegraphics[width=0.3\textwidth]{newfigures/a_ChemChem_BioSnap}%
    %\text{
    \end{minipage}
    \begin{minipage}{\marginparwidth}
    \text{Motivating social.}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{newfigures/a_ChemChem_BioSnap}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{newfigures/a_ChemChem_BioSnap}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{newfigures/a_ChemChem_BioSnap}%
  \end{minipage}\\%
   \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{newfigures/a_ChemChem_BioSnap}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{newfigures/a_ChemChem_BioSnap}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{newfigures/a_ChemChem_BioSnap}%
  \end{minipage}\\%
  \caption{Results of the wedges experiment on six real-world networks from
    Table~\ref{tab:datasets}. Pair-seeded PageRank and TRPR produce superior
    results as compared to single-seeded PageRank in all experiments.}
  \label{fig:newfigures}
\end{figure}
\end{fullwidth} 


\begin{figure}[t]
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-wedges-edges/a_Penn94_wedge_edge}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-wedges-edges/a_MU_wedge_edge}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-wedges-edges/a_caltech_wedges_edges}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-wedges-edges/a_CC_wedge_edge}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-wedges-edges/a_PP_wedge_edge}%
  \end{minipage}\\%
  \begin{minipage}{.99\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-wedges-edges/a_email_wedges_edges}%
  \end{minipage}\\%
  \caption{Results of the wedges experiment on six real-world networks from
    Table~\ref{tab:datasets}. Pair-seeded PageRank and TRPR produce superior
    results as compared to single-seeded PageRank in all experiments.}
  \label{fig:real-wedges-edges}
\end{figure}

\begin{figure}[t]
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_penn_80_20}%
  \end{minipage}\\%
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_MU_80_20}%
  \end{minipage}\\%
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_caltech_80_20}%
  \end{minipage}\\%
  \caption{Results of the 80-20 experiments on the three Facebook100 networks.
    AA and JS produce the best results on Penn94 and MU78.  These local methods
    give comparable results compared to TRPR and pair-seeded PageRank on the
    Caltech36 network. Pair-seeded PageRank and TRPR still outperform
    single-seeded PageRank.}
  \label{fig:facebook100}
\end{figure}

\begin{figure}[t]
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_drug_80_20}%
  \end{minipage}\\%
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_protein_80_20}%
  \end{minipage}\\%
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_email_80_20}%
  \end{minipage}\\%
  \caption{Results of the 80-20 experiment on the biological and email networks.
    The small inset in the email figure in the bottom panel is a zoom-in on the
    values from 0.9 to 1 for the first four methods. PA can perform better than
    diffusion type methods on protein-protein interaction networks; however,
    this result agrees with the literature showing that such networks evolve
    preferentially.}
  \label{fig:nonfacebook}
\end{figure}
}


%%%%%%%% OLD VERSION
\hide{
\subsection{Real world graphs}
\label{sec:real-world}
In this section we consider 6 real world graphs coming from different domains and we perform the task of pairwise link prediction. We use Biology datasets from the BioSNAP datasets~\cite{biosnapnets}, three Facebook100 datasets from~\cite{Traud-facebook100-2011}, and an email communication network from~\cite{Guimer-selfsimilar-2003}. We provide some statistics about these datasets in Table~\ref{tab:datasets}.

\begin{table}
\caption{Statistics or the real world datasets used in this paper}\vspace{-0.5\baselineskip}
	\label{tab:datasets}
	\begin{tabularx}{\linewidth}{lXXX}
	\toprule
	 Network name &  nodes & edges & type\\
	 \midrule
	  Penn94 &  41536 & 1362220 & Social \\
	  MU78 &  15425 & 649441 & Social \\
	  Caltech36 &  762 & 16651 & Social \\
	  Ch-Ch-Miner &  1510 & 48512 & Biology \\
	  P-P-Pathways &  21521 & 338624 & Biology\\
	  email &  1133 & 5451 & Communication\\
	  CollegeMsg &  1899 & 13838 & Temporal\\
	  \bottomrule
		\end{tabularx}
\end{table}

The wedges experiment results are shown in Figure~\ref{fig:real-wedges-edges}, and it is clear that pair-seeded PageRank and TRPR consistently produce better performance as compared to single seeded PageRank. We show the 80-20 experiments results on the social networks we use in figure~\ref{fig:facebook100}. Here, we observe an interesting improvement of local methods such as Adamic-Adar and Jaccard Similarity. Nevertheless, this is not unexpected, as these metrics model the social interactions paradigm such as having a large number of common friends [XXX research evidence?]. We show the 80-20 experiment on the remaining non social networks in Figure~\ref{fig:nonfacebook}. The one scenario in which a local method outperforms the diffusion type methods is the Protein-Protein interaction network where the PA metric produces the best performance. Nevertheless, this comes as no surprise as studies have suggested that preferential attachment governs the PPI networks evolution~\cite{Eisenberg-PPIprefattach-2003,Jin-PPIevolution-2013}. 

\begin{figure}
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.49\linewidth]{real-wedges-edges/a_Penn94_wedge_edge}%
		\includegraphics[width=0.49\linewidth]{real-wedges-edges/a_CC_wedge_edge}%
	\end{minipage}\\
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.49\linewidth]{real-wedges-edges/a_MU_wedge_edge}%
		\includegraphics[width=0.49\linewidth]{real-wedges-edges/a_PP_wedge_edge}%
	\end{minipage}\\
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.49\linewidth]{real-wedges-edges/a_caltech_wedges_edges}%
		\includegraphics[width=0.49\linewidth]{real-wedges-edges/a_email_wedges_edges}%
	\end{minipage}
	\caption{This is the wedges experiment on the 6 real world networks from table~\ref{tab:datasets}. Pair-seeded PageRank and TRPR produce superior results as compared to single-seeded PageRank in all experiments.}
	\label{fig:real-wedges-edges}
\end{figure}

\begin{figure}
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_penn_80_20}%
	\end{minipage}\\%
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_MU_80_20}%
	\end{minipage}\\%
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_caltech_80_20}%
	\end{minipage}\\%
	\caption{This is the 80-20 experiment on the social networks from the real world graphs we are testing our methods on. AA and JS produce the best results on two of the networks and comparable results to TRPR and pair-seeded PageRank on the third network. Since the AA and JS measures, it is no surprise that they can produce better results tha diffusion type methods. Further, Pair-seeded PageRank and TRPR remain to outperform single-seeded PageRank.}
	\label{fig:facebook100}
\end{figure}



\begin{figure}
		\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_drug_80_20}%
	\end{minipage}\\%
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_protein_80_20}%
	\end{minipage}\\%
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_email_80_20}%
	\end{minipage}\\%
	\caption{The 80-20 experiment on the non-social network type graphs from table~\ref{tab:datasets}. The small inset figure in the bottom panel is a zoom-in on the values from 0.9 to 1 for the first 4 methods. One interesting observation to note here is that PA can perform better than diffusion type methods on PPI networks, nevertheless, research evidence has shown that PPI networks evolve preferentially, and this result agrees with the literature as PA shows the best results on the PPI network.}
	\label{fig:nonfacebook}
\end{figure}
}



%In all 80-20 experiments Pa
%
%One scenario in which diffusion methods do not perform well in general is the PPI
%
%The preferential attachment method performs very well on the protein-protein interaction network (middle panel of Figure~\ref{fig:nonfacebook}), and this is not unexpected too, 
%
%\xhdr{Final remarks on real networks} We observed in this section that pair-seeded PageRank and TRPR are consistently better the single-seeded PageRank diffusion method. We also observed that in certain scenarios local methods can be superior (AA and JS on social networks and PA on Protein-Protein interaction network), but this came as no surprise as studies have suggested that the natural evolution of PPI networks is in a preferential attachment manner
%
%or , but this came as no surprise as 
%
%
%pair-seeded PageRank and TRPR can perform worse than the simple local methods in select scenarios. But this comes as no big surp
%
%we also observed that simple local methods such as Adamic-Adar and Jaccard Similarity are powerful on social networks, and 
%
%
%Additionally, we can still observe that pair-seeded PageRank and TRPR 
%
%
%The protein-protein interaction networks and the drug-drug interaction networks reveal high scores for the preferential attachment method, 
%
%
%
%
%and what this indicates is that a well known pair of proteins is higly lig


==> 005-03-temporal.tex <==
\subsection{Case study on a temporal graph}
As stated in the introduction, link prediction can be viewed as the task
of predicting missing links from the network or future hidden links. With our
wedges and 80-20 experiments, we modeled the prediciton task of missing
links. Next, we intend to focus on a case study of predicting future links on a
communication network. We use the temporal network CollegeMsg~\cite{Panzarasa-college-2009},
which has timestamped edges between students on a college's private messaging service.
The summary statistics of the dataset are in Table~\ref{tab:datasets}.

We run the 80-20 experiment on this network while treating the earliest $80\%$
of the unique edges as our training data and the remainder in the test data. We use two evaluations here:
\begin{itemize}
\item The ``AND'' metric (top panel of Figure~\ref{fig:collegemsg}) considers
  predictions on nodes where both edges connecting the node to the seed edge are
  in the test data.
\item The ``OR'' metric (bottom panel of Figure~\ref{fig:collegemsg}) considers
  predictions on nodes where exactly one of the two edges connecting the node to
  the seed edge appears in the test data.
\end{itemize}
Figure~\ref{fig:collegemsg} shows that our pair-seeded PageRank and
TRPR outperform all the other link prediction metrics, and thus, both pair-seeded
PageRank and TRPR are well suited for pairwise link prediciton on temporal
networks.

\hide{
\begin{figure}[t]
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_college_msg_and}%
  \end{minipage}\\%
  \begin{minipage}{.49\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{real-80-20/aa_college_msg_or}%
  \end{minipage}\\%
  \caption{The 80-20 experiment applied on the CollegeMsg temporal network where
    training and test data are split by edge arrival time.  The ``AND'' metric
    (top panel) measures pairwise link prediction performance for triangles
    where both edges connecting the predicted node to the seed edge are in the
    test data.  The ``OR'' metric (bottom panel) measures performance where only
    one of the two triangle edges connecting the predicted node to the seed edge
    is in the test data.  The ``AND'' metric is more challenging, and
    performance is generally worse compared to the ``OR'' metric. Regardless, in
    both cases, our pair-seeded PageRank and TRPR methods have the best
    prediction performance.}
  \label{fig:collegemsg}
\end{figure}
}



%%%%%%%%%% OLD VERSION
\hide{
\subsection{Case study on a temporal graph}
As stated in the Introduction section, link prediction can be viewed as the task of predicting missing links from the network or future hidden links. With our wedges and 80-20 experiments, we model the prediciton task of missing links. Here, we intend to focus on a case study of predicting future links on a communication network. We use the temporal network CollegeMsg from SNAP~\cite{snapnets} and show its statistics in table~\ref{tab:datasets}.

We run the 80-20 experiment on this network while treating the earliest $80\%$ of the unique edges as our training data. We use two evaluations here and show the results in Figure~\ref{fig:collegemsg}
\begin{itemize}
\item The OR metric (bottom panel of Figure~\ref{fig:collegemsg}) is the one we have been using so far in this paper and it considers a node prediction correct if it was connected to the seed edge by \textit{at least} one edge in the testing data.
\item The AND metric (top panel) considers a node prediction correct if it forms a triangle with the seed edge in the testing data. 
\end{itemize}

Figure~\ref{fig:collegemsg} show shows that our two methods pair-seeded PageRank and TRPR outperform all the othe link prediction metrics, and thus, both pair-seeded PageRank and TRPR are well suited for pairwise link prediciton on temporal networks.

\begin{figure}
		\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_college_msg_and}%
	\end{minipage}\\%
	\begin{minipage}{.49\textwidth}
	\centering
		\includegraphics[width=0.99\linewidth]{real-80-20/aa_college_msg_or}%
	\end{minipage}\\%
	\caption{The 80-20 experiment applied on the CollegeMsg network after treating the first $80\%$ of the unique set of edges as training data, and the remaining edges for verification. We use two evaluations here. The OR metric (bottom panel) is the one we have been using so far in this paper and it considers a node prediction correct if it was connected to the seed edge by \textit{at least} one edge in the testing data. The AND metric (top panel) considers a node prediction correct if it forms a triangle with the seed edge in the testing data. The latter metric is the more challenging one, and hence we would expect each method's results to perform worse in the AND metric. In both evaluation metrics, we can conclude that pair-seeded PageRank and TRPR are the best performing and are well suited for making predictions on a temporal networlk.}
	\label{fig:collegemsg}
\end{figure}
}


%In this section we bring our attention back to the standard link prediction problem. We show how the methods we presented in this paper can be used to further enhance link prediction results. We design our experiment as follows. For a given graph, we split the graph $\mA$ into training and testing data $\mA_{train}$ and $\mA_{test}$ while using $80\%$ of the edges from the original graph in the training graph (in the scenario of the temporal network CollegeMsg, we take the first $80\%$ of the set of unique edges to be in our training data). Then, for the nodes corresponding to the top $100$ degree nodes, we perform seeded PageRank as a baseline method for link prediction. We evaluate the result with $\mA_{test}$ being our ground truth hidden edges, and consider the resulting AUC scores our baseline measures. Note that the choice of the top $100$ nodes only serves the purpose of identifying nodes that have a higher chance of having connections in the testing data. Then, we will use four methods inspired by our pairwise link prediction methods to perform the standard link prediction task. We summarize them below.
%\begin{enumerate}
%%\item i 
%\item  [sum\textcolor{plots1}{$\blacktriangle$}] For a certain node $i$, aggregate the pair-seeded PageRank results from all edges adjacent to $i$. This is equivalent to performing PageRank with a normalized initial vector valued $1$ at the indices of all the neighbors of $i$, and $degree(i)$ at index $i$.
%\item [max\textcolor{plots2}{$\bullet$}] This is similar to the previous approach, but here, we instead take the element-wise maximum value of the pair-seeded PageRank vectors.
%\item [star-seed\textcolor{plots3}{\arc}] This is similar to pair-seeded PageRank, except that the starting vector has a nonzero structure at $i$, its seed node index, and the indices of all its neighbors, and its value is $1/degree(i)$.
%\item [TRPR\textcolor{plots4}{$\blacklozenge$}] This uses the same starting vector used by star-seed, but instead, applies the TRPR algorithm on it.
%\end{enumerate}
%\xhdr{Neigborhood link prediction} All of these methods fall under the category of using a node's neighborhood for the purpose of predicting its links. We use four of the previously described networks in Section~\ref{sec:real-world}, and present our results in Figure~\ref{fig:linkpred}. These results suggest that neighborhood link prediction methods are superior to seeded PageRank as a link prediction method.
%
%%\begin{figure}
%%	\begin{minipage}{.49\textwidth}
%%	\centering
%%		\includegraphics[width=0.49\linewidth]{linkpred/a_caltech_links}
%%		\includegraphics[width=0.49\linewidth]{linkpred/a_cc_links}
%%	\end{minipage}\\%
%%	\begin{minipage}{.49\textwidth}
%%	\centering
%%		\includegraphics[width=0.49\linewidth]{linkpred/a_college_msg_links}
%%		\includegraphics[width=0.49\linewidth]{linkpred/a_email_links}
%%	\end{minipage}
%%	\caption{A standard link prediction experiment over 4 real-world graphs. The scatter plot shows the link prediction AUC results of 100 experiments of methods inspired by our pairwise link prediction proposal against the AUC scores of seeded PageRank. The solid black line is the plot of $f(x) = x$. We see that in most cases the four methods outperform the classical seeded PageRank method. This study suggests that it is likely useful to consider a node's neighborhood for the purposes of link prediction with PageRank.}
%%	\label{fig:linkpred}
%%\end{figure}


==> dgleich-extra.tex <==
\usepackage{ushort}
\newcommand{\cel}[1]{\ushort{#1}}
\newcommand{\cbmat}[1]{\left\{ \begin{matrix} #1 \end{matrix} \right\}}
\newcommand{\csbmat}[1]{\left\{\! \begin{smallmatrix} #1
\end{smallmatrix} \! \right\}}
%\newcommand{\csbmat}[1]{\underline{\sbmat{#1}}}
\newcommand{\smallmath}[1]{\begin{smallmatrix}#1\end{smallmatrix}}
\newcommand{\celm}[1]{\cel{\mat{#1}}}
\newcommand{\celv}[1]{\cel{\vec{#1}}}



\newcommand{\calpha}{\ensuremath{\cel{\alpha}}}
\newcommand{\cbeta}{\ensuremath{\cel{\beta}}}
\newcommand{\clambda}{\ensuremath{\cel{\lambda}}}

\newcommand{\cone}{\ensuremath{\cel{1}}}
\newcommand{\ca}{\ensuremath{\cel{a}}}
\newcommand{\cb}{\ensuremath{\cel{b}}}
\newcommand{\cc}{\ensuremath{\cel{c}}}
\newcommand{\cd}{\ensuremath{\cel{d}}}
\newcommand{\ce}{\ensuremath{\cel{e}}}
\newcommand{\cf}{\ensuremath{\cel{f}}}
\newcommand{\cg}{\ensuremath{\cel{g}}}
\newcommand{\ch}{\ensuremath{\cel{h}}}
\newcommand{\ci}{\ensuremath{\cel{i}}}
\newcommand{\cj}{\ensuremath{\cel{j}}}
\newcommand{\ck}{\ensuremath{\cel{k}}}
\newcommand{\cl}{\ensuremath{\cel{l}}}
\newcommand{\cm}{\ensuremath{\cel{m}}}
\newcommand{\cn}{\ensuremath{\cel{n}}}
\newcommand{\co}{\ensuremath{\cel{o}}}
\newcommand{\cp}{\ensuremath{\cel{p}}}
\newcommand{\cq}{\ensuremath{\cel{q}}}
%\newcommand{\cr}{\ensuremath{\cel{r}}}
\newcommand{\cs}{\ensuremath{\cel{s}}}
\newcommand{\ct}{\ensuremath{\cel{t}}}
\newcommand{\cu}{\ensuremath{\cel{u}}}
\newcommand{\cv}{\ensuremath{\cel{v}}}
\newcommand{\cw}{\ensuremath{\cel{w}}}
\newcommand{\cx}{\ensuremath{\cel{x}}}
\newcommand{\cy}{\ensuremath{\cel{y}}}
\newcommand{\cz}{\ensuremath{\cel{z}}}


\newcommand{\cA}{\ensuremath{\cel{A}}}
\newcommand{\cB}{\ensuremath{\cel{B}}}
\newcommand{\cC}{\ensuremath{\cel{C}}}
\newcommand{\cD}{\ensuremath{\cel{D}}}
\newcommand{\cE}{\ensuremath{\cel{E}}}
\newcommand{\cF}{\ensuremath{\cel{F}}}
\newcommand{\cG}{\ensuremath{\cel{G}}}
\newcommand{\cH}{\ensuremath{\cel{H}}}
\newcommand{\cI}{\ensuremath{\cel{I}}}
\newcommand{\cJ}{\ensuremath{\cel{J}}}
\newcommand{\cK}{\ensuremath{\cel{K}}}
\newcommand{\cL}{\ensuremath{\cel{L}}}
\newcommand{\cM}{\ensuremath{\cel{M}}}
\newcommand{\cN}{\ensuremath{\cel{N}}}
\newcommand{\cO}{\ensuremath{\cel{O}}}
\newcommand{\cP}{\ensuremath{\cel{P}}}
\newcommand{\cQ}{\ensuremath{\cel{Q}}}
\newcommand{\cR}{\ensuremath{\cel{R}}}
\newcommand{\cS}{\ensuremath{\cel{S}}}
\newcommand{\cT}{\ensuremath{\cel{T}}}
\newcommand{\cU}{\ensuremath{\cel{U}}}
\newcommand{\cV}{\ensuremath{\cel{V}}}
\newcommand{\cW}{\ensuremath{\cel{W}}}
\newcommand{\cX}{\ensuremath{\cel{X}}}
\newcommand{\cY}{\ensuremath{\cel{Y}}}
\newcommand{\cZ}{\ensuremath{\cel{Z}}}


\newcommand{\cva}{\ensuremath{\celv{a}}}
\newcommand{\cvb}{\ensuremath{\celv{b}}}
\newcommand{\cvc}{\ensuremath{\celv{c}}}
\newcommand{\cvd}{\ensuremath{\celv{d}}}
\newcommand{\cve}{\ensuremath{\celv{e}}}
\newcommand{\cvf}{\ensuremath{\celv{f}}}
\newcommand{\cvg}{\ensuremath{\celv{g}}}
\newcommand{\cvh}{\ensuremath{\celv{h}}}
\newcommand{\cvi}{\ensuremath{\celv{i}}}
\newcommand{\cvj}{\ensuremath{\celv{j}}}
\newcommand{\cvk}{\ensuremath{\celv{k}}}
\newcommand{\cvl}{\ensuremath{\celv{l}}}
\newcommand{\cvm}{\ensuremath{\celv{m}}}
\newcommand{\cvn}{\ensuremath{\celv{n}}}
\newcommand{\cvo}{\ensuremath{\celv{o}}}
\newcommand{\cvp}{\ensuremath{\celv{p}}}
\newcommand{\cvq}{\ensuremath{\celv{q}}}
\newcommand{\cvr}{\ensuremath{\celv{r}}}
\newcommand{\cvs}{\ensuremath{\celv{s}}}
\newcommand{\cvt}{\ensuremath{\celv{t}}}
\newcommand{\cvu}{\ensuremath{\celv{u}}}
\newcommand{\cvv}{\ensuremath{\celv{v}}}
\newcommand{\cvw}{\ensuremath{\celv{w}}}
\newcommand{\cvx}{\ensuremath{\celv{x}}}
\newcommand{\cvy}{\ensuremath{\celv{y}}}
\newcommand{\cvz}{\ensuremath{\celv{z}}}

\providecommand{\cmA}{\ensuremath{\celm{A}}}
\providecommand{\cmB}{\ensuremath{\celm{B}}}
\providecommand{\cmC}{\ensuremath{\celm{C}}}
\providecommand{\cmD}{\ensuremath{\celm{D}}}
\providecommand{\cmE}{\ensuremath{\celm{E}}}
\providecommand{\cmF}{\ensuremath{\celm{F}}}
\providecommand{\cmG}{\ensuremath{\celm{G}}}
\providecommand{\cmH}{\ensuremath{\celm{H}}}
\providecommand{\cmI}{\ensuremath{\celm{I}}}
\providecommand{\cmJ}{\ensuremath{\celm{J}}}
\providecommand{\cmK}{\ensuremath{\celm{K}}}
\providecommand{\cmL}{\ensuremath{\celm{L}}}
\providecommand{\cmM}{\ensuremath{\celm{M}}}
\providecommand{\cmN}{\ensuremath{\celm{N}}}
\providecommand{\cmO}{\ensuremath{\celm{O}}}
\providecommand{\cmP}{\ensuremath{\celm{P}}}
\providecommand{\cmQ}{\ensuremath{\celm{Q}}}
\providecommand{\cmR}{\ensuremath{\celm{R}}}
\providecommand{\cmS}{\ensuremath{\celm{S}}}
\providecommand{\cmT}{\ensuremath{\celm{T}}}
\providecommand{\cmU}{\ensuremath{\celm{U}}}
\providecommand{\cmV}{\ensuremath{\celm{V}}}
\providecommand{\cmW}{\ensuremath{\celm{W}}}
\providecommand{\cmX}{\ensuremath{\celm{X}}}
\providecommand{\cmY}{\ensuremath{\celm{Y}}}
\providecommand{\cmZ}{\ensuremath{\celm{Z}}}

\newcommand{\cmPt}{\cel{\mat{\tilde{P}}}}
\renewcommand{\cmPt}{\mat{\tilde{P}}}

\newcommand{\elm}[1]{\cel{#1}}
